Generating natural images with direct Patch Distributions Matching

Many traditional computer vision algorithms generate realistic images by requiring that each patch in the generated image be similar to a patch in a training image and vice versa. Recently, this classical approach has been replaced by adversarial training with a patch discriminator. The adversarial approach avoids the computational burden of finding nearest neighbors of patches but often requires very long training times and may fail to match the distribution of patches. In this paper we leverage the recently developed Sliced Wasserstein Distance and develop an algorithm that explicitly and efficiently minimizes the distance between patch distributions in two images. Our method is conceptually simple, requires no training and can be implemented in a few lines of codes. On a number of image generation tasks we show that our results are often superior to single-image-GANs, require no training, and can generate high quality images in a few seconds. Our implementation is available at https://github.com/ariel415el/GPDM

==> Generating Natural Images with Direct Patch Distributions Matching [ECCV]/images/0_Teaser_Figure.tex <==
\begin{figure}[H]
    \makebox[\textwidth][c]{\includegraphics[width=1\textwidth]{images/0_Teaser_Figure.jpg}}%
    % \includegraphics[width=1\linewidth]{images/0_Teaser_Figure.jpg}
    \caption{By efficiently matching the distribution of patches between images we can solve a broad spectrum of single-image generative tasks without training a per-image GAN or computing patch nearest neighbors.}
   \label{fig:Teaser}
\end{figure}

==> Generating Natural Images with Direct Patch Distributions Matching [ECCV]/images/3_Overview.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{images/3_Overview.jpg}
    \caption{{\bf Left:} GPDM’s multi-scale architecture: At each scale, $i$, an image is optimized to have similar patch distribution as the target $x_i$. {\bf Right:} The generation module $G$  is an optimization process of the differentiable patch-distribution metric $SWD(x,y)$. Triangles marked with \textbf{R} stand for up/downscale.}
    \label{fig:Overview}
\end{figure}


==> Generating Natural Images with Direct Patch Distributions Matching [ECCV]/images/4_Reshuffling.tex <==
\begin{figure}[hb]
    \centering
    \includegraphics[width=\linewidth]{images/4_Reshuffling.jpg}
    \caption{Image reshuffling on images from the Places50 and SIGD16 selected by~\cite{GPNN}.}
\label{fig:Reshuffling}
\end{figure}

==> Generating Natural Images with Direct Patch Distributions Matching [ECCV]/images/4_Retargeting.tex <==
\begin{figure}
 \centering
    \includegraphics[width=0.9\textwidth]{images/4_Retargeting.jpg}
    \caption{Image retargeting results.}
    \label{fig:Retargeting}
\end{figure}

==> Generating Natural Images with Direct Patch Distributions Matching [ECCV]/images/4_Style_Transfer.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{images/4_Style_Transfer.jpg}
    \caption{Style/texture transfer: Each image triplet shows a content image, a style/texture image and the results of combining them with our synthesis method.}
\label{fig:Style_Transfer}
\end{figure}

==> Generating Natural Images with Direct Patch Distributions Matching [ECCV]/images/8_HQ_style.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{images/8_HQ_style.jpg}
    \caption{High resolution style transfer images generated (a) GPNN(no-$\alpha$) with approximate nearest neighbor  ($\sim70$ seconds, GPU), (b) GPNN($\alpha$=0.005) with exact nearest neighbor ($\sim1900$ seconds, GPU). (c) Our result ($\sim60$ seconds, GPU). $\alpha$ is the completeness enforcing parameter and no-$\alpha$ means no constraint.}
    \label{fig:HQ_images}
\end{figure}


==> Generating Natural Images with Direct Patch Distributions Matching [ECCV]/other/Algorithm.tex <==
\begin{algorithm}[H]
    % \captionof{algorithm}{GPDM Module} 
    \hspace*{\algorithmicindent} \textbf{Input}: Target image x, initial guess $\hat{y}$, \\
    \hspace*{\algorithmicindent} learning rate $\beta$  \\
    \hspace*{\algorithmicindent} \textbf{Output}: Optimized image y
    \begin{algorithmic}[1]
        \State $y\leftarrow\hat{y}$
        \While{not converged}
         \State $L \leftarrow 0$
          \For{i=1,k}
            \State $\omega\sim N(0,\sigma I)$ 
            \State $\omega\leftarrow unflat(\frac{\omega}{\|w\|})$
            \State $p\leftarrow flat(conv2d(x,\omega))$
            \State $q\leftarrow flat(conv2d(y,\omega))$
            \State $L\leftarrow L+ \frac{1}{k} |sort(p) -  sort(q)|$ 
            \EndFor
            \State $y\leftarrow y- \beta\nabla_{y}L$
        \EndWhile
    \end{algorithmic} 
\caption[]{A pseudo-code of the GPDM module where SWD over sets of patches in two images is computed and differentiated through. The "flat/unflat" operators reshapes a tensor into a vector and vice-versa.}
\label{algorithm-1}
\end{algorithm}



==> Generating Natural Images with Direct Patch Distributions Matching [ECCV]/other/results_table.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{|c|c|c|c|c|c|c|c|}
    %\toprule
    \hline
    Dataset & Method & SFID$\downarrow$ & Diversity$\uparrow$ & Dataset & Method & SFID$\downarrow$  & Diversity$\uparrow$  \\
   % \midrule
   \hline
    \multirow{3}{*}{Places5} & Ours & 0.068 & 0.56 & \multirow{3}{*}{SIGD16} & Ours & 0.069  & 0.67\\
     & GPNN & 0.065 & 0.5  & & GPNN & 0.122 & 0.52 \\
     & SINGAN & 0.082 & 0.5  & & SINGAN & 0.172 & 0.49 \\ 

    %\bottomrule
    \hline
    \end{tabular}
    \caption[]{Qualitative Comparison image-reshuffling.}
    \label{tab:Reshuffling results}
\end{table}

==> Generating Natural Images with Direct Patch Distributions Matching [ECCV]/other/timing_table.tex <==
\begin{tabular}{ |c | c | c | c | c | c |}
    \hline
    image-size & $64^2$ & $128^2$ & $256^2$ & $512^2$ & $1024^2$ \\
    \hline
    SWD(64) & 0.002 & 0.006 & 0.021 & 0.086 & 0.335\\
    NN-exact & 0.086 & 0.110 & 0.336 & 4.144 & 73.23\\
    NN-IVF& 0.101 & 0.137 & 0.382 & 1.082 & 5.530\\
    \hline
\end{tabular}
\captionof{table}{Compute time (seconds) of SWD (64 projections), exact nearest neighbor (FaissFlat) and approximated nearest neighbor (Inverted Index with $\sqrt{M}$ bins where M is the number of patches) for different image sizes. All computation are done on a NVIDIA TITAN X GPU.}
\label{tab:timing_table}

